MPC-guided Imitation Learning of Neural Network Policies for the Artificial Pancreas

Even though model predictive control (MPC) is currently the main algorithm for insulin control in the artificial pancreas (AP), it usually requires complex online optimizations, which are infeasible for resource-constrained medical devices. MPC also typically relies on state estimation, an error-prone process. In this paper, we introduce a novel approach to AP control that uses Imitation Learning to synthesize neural-network insulin policies from MPC-computed demonstrations. Such policies are computationally efficient and, by instrumenting MPC at training time with full state information, they can directly map measurements into optimal therapy decisions, thus bypassing state estimation. We apply Bayesian inference via Monte Carlo Dropout to learn policies, which allows us to quantify prediction uncertainty and thereby derive safer therapy decisions. We show that our control policies trained under a specific patient model readily generalize (in terms of model parameters and disturbance distributions) to patient cohorts, consistently outperforming traditional MPC with state estimation.

==> acknowledgment.tex <==
\section*{Acknowledgment}

Research supported in part by %
.



==> author.tex <==


\author{\IEEEauthorblockN{1\textsuperscript{st} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{2\textsuperscript{nd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{3\textsuperscript{rd} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{4\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{5\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
\and
\IEEEauthorblockN{6\textsuperscript{th} Given Name Surname}
\IEEEauthorblockA{\textit{dept. name of organization (of Aff.)} \\
\textit{name of organization (of Aff.)}\\
City, Country \\
email address}
}

==> background.tex <==
% \section{Background} \label{sec:background}

% \subsection{Disturbance}

% A major kind of disturbance in the control of diabetes patients' BG is the meals they have. The uncertainty in the ingredient, amount and time of the meals is a huge challenge for artificial pancreas system designs. In this paper, we denote $\disturbance_t$ as the amount (in gram) of the carbohydrate a patient ingests at time $t$.

% \subsection{Patient Model}

% Mathematical modelling of homeostatic systems has
% long held great promise to explain the behaviour of closed loop physiological systems. Many mathematical models have been developed by researchers to better understand the mechanisms of the glucose-insulin regulatory system~\cite{bergman1979quantitative,chen2015towards,hovorka2004nonlinear,wach1995numerical,sturis1991computer,bleckert1998mixed,rao2003constrained}. We consider the nonlinear ODE model proposed by Jacobs et al.~\cite{resalat2016design}, which is an extension of the well-established model proposed by Hovorka~\cite{hovorka2004nonlinear}, as the patient model.  It describes the dynamics between insulin and blood glucose level in a type 1 diabetes patient, such as their absorption, metabolism, excretion and transport between different body compartments (e.g., kidney, subcutaneous compartment). This glucoregulatory model consists of a glucose kinetics model, insulin kinetics and dynamics models, and glucagon kinetics and dynamics models. It can also describe the dynamics of a dual-hormone glucose model with insulin and glucagon, which is antagonistic to  insulin that protects against hypoglycemia, and capture the effect of exercises on BG. However, in our paper, we use a single hormone patient model and does not consider the existence of exercises because insulin and meals are the most important regulatory hormone and disturbance for BG. We adopt the model parameter distributions in~\cite{paoletti_arxiv} to samples different parameter for each patient to build a patient cohort. The parameters of each patient are also oscillating through time to represent the intra-patient variation phenomena.

% At time $t$, the inputs of the patient model is the insulin infusion rate in the unit of ($mU/min$) the disturbance is the amount of CHO the patient ingests in the unit of ($gram$). We denote them as $u^t$ and $D_G^t$, respectively. The following equations describe the model dynamics and the output function:

% \begin{align}
% \dot{\mathbf{x}}_t = ~& {\bf F}\left(\mathbf{x}_t, u_t, \disturbance_t \right), \ t\in\mathbb{Z}^{\geq 0}
% \label{eq:state_space_form}\\
% % y(t) = & h\left(\mathbf{x}(t)\right) + \hongkai{\epsilon^k} \label{eq:output}
% y_t = ~& h\left(\mathbf{x}_t\right)+\epsilon_t, \ t\in\mathbb{Z}^{\geq 0} \label{eq:output}
% \end{align}

% where $x$ is the 14-dimensional system state, $y$ is the output of the model, which is the CGM sensor measurements, and $\epsilon$ is the sensor noise. The evolution of the system is given by the continuous ODE equations {\bf F} at time $t$, and the sensor measurements are measured using the output function $h$ at discrete time $k$. The sensor noise $\epsilon$ is Gaussian. 

% The patient model consists of the following subsystems.

% We denote the upper and lower bounds of the healthy range for human blood glucose concentration are $BG_{ub}$ and $BG_{lb}$, which are 180 ml/dL and 70 ml/dL, respectively.

% \subsection{Model Predictive Control}

% Model predictive control is a process control technique that uses system model to predict and optimize the control actions to minimize some cost functions under certain constraints.

% \subsection{Imitation Learning}

% Imitation learning is a category of machine learning algorithms that aims at improve performance by mimicking demonstrations from a teacher~\cite{osa2018algorithmic}. The two major types of imitation learning algorithms are behavioral cloning and inverse reinforcement learning. Behavioral cloning directly maps from features to trajectories/actions as the description of the policy without recovering the reward function. In contrast, inverse reinforcement learning encoded the policy as the solution of an optimization or planning problem, and learns a (surrogate) cost function so that the behavior that results from solving that optimization is in some sense like that demonstrated by the expert.

% Imitation learning algorithms are commonly used to solve sequential control problems.
% \subsection{Policy Search}





==> system.tex <==
% \section{System Overview} \label{sec:system}

% \hc{This section describe the system we propose, the PLATO+dropout algorithm to search a stochastic control policy. }

% {\color{orange} SL: we need to introduce the training phase and the deployment phase, and their challenges and settings respectively.}

% \np{``supervised policy'' is called actually ``supervision policy''. the notations $\superviseMPC$ and $\teacherMPC$ are a bit cumbersome; why don't we just use notations $\pi^*$ and $\pi_{\rho}^i$?}

% \np{also, instead of calling it all the time ``adaptive trajectory optimization'', let's just call it PLATO}

% \hc{After all, PLATO is the title of another paper, should we just use it? Also, we have different algorithm, policy representations, and policy learning methods.}

% The flowchart of the training phase in our proposed algorithm is illustrated in Fig.~\ref{fig:systemOverview}. The system contains the following components:
% \begin{itemize}
%     \item Plant: A virtual patient is represented by a mathematical model ${\bf F_\lambda}$ with parameters $\lambda$. At time $t$, the next state $\dot{\mathbf{x}}_{t+1}$ is determined by the current state $\dot{\mathbf{x}}_t$, the insulin injection $u_t$ and the disturbance $\disturbance_t$.
%     \item Disturbance: At time $t$, we sample the meal disturbance $\disturbance_t$ from some distribution $P(\disturbance)$.
%     \item Supervised policy $\superviseMPC$: At time $t$, its inputs are $x_t$, and future meals $d_{t,\cdots,t+\predh}$ and its output is the optimal insulin amount $\actionSuperviseMPC$, which is stored in the training dataset $S$. It conduct trajectory optimization to minimizes a cost function, i.e., the sum of discrepancy between the predicted BG and target BG and the discrepancy between consecutive insulin injections. 
%     \item Adaptive teacher policy $\teacherMPC$: At time $t$, its output is $\actionTeacherMPC$, and inputs are $x_t$, $d_{t,\cdots,t+\predh}$ and $\actionControlpolicy$. It minimizes both the cost function of $\superviseMPC$ and the discrepancy between the decision variable $\actionTeacherMPC$ (i.e., the next insulin injection) and the output of the current half-trained control policy $\actionControlpolicy$ in an adaptive manner. 
%     \item Learner policy $\controlpolicy
%     $: It is represented by a recurrent neural network with parameters $\theta$. At time $t$, it computes an insulin injection amount $\actionControlpolicy$ based on the its internal state $s^L_t$, latest CGM measurement $y_t$, latest insulin injection provided to the patient $\actionTeacherMPC$ and a future meal $\disturbance_{t+\predh}$.
%     \item Training dataset $S$: It collects CGM measurement sequence $y_{1, \cdots, t}$, insulin injection amount sequence $u_{1, \cdots, t}$ and meal sequence $d_{1,\cdots,t+\predh}$ as the input vectors. The corresponding outputs are the optimal insulin amount computed by $\superviseMPC$. The Learner policy $\controlpolicy$ is trained on $S$ using a supervised learning method periodically.
% \end{itemize}

% A fundamental challenge for is the construction of the training dataset needs to well represent the state space $\controlpolicy$ is going to enter in order to mitigate the Covariate Shift problem. In our design, with the interaction between $\teacherMPC$ and $\controlpolicy$, we avoid both randomly exploring all possible state spaces which is experience expensive and time consuming, and directly training with trajectories guided by an MPC controller which does not explore state spaces that $\controlpolicy$ is likely to visit in test time because of external disturbance and decision errors. For the meal $\disturbance_t$, previous work~\cite{hughes2011anticipating} is able to develop a control law to anticipate a meal given a probabilistic description of the patient's meal behavior. Some smartphone applications~\cite{OnTrack} have showed the ability for future meal predictions for type 1 diabetes patients. In our work, the knowledge of the meal prediction is not the focus. For this reason, we assume all the onset time and carbohydrate amount of the meals $d_{1,...,\infty}$ are given later in this paper.

% \begin{figure}[tbp]
% \centerline{\includegraphics[width= 0.5\textwidth]{img/systemOverview6.PNG}}
% \caption{Overview of artificial pancreas control policy algorithm in training phase at time $t$. \np{why some arrows are orange? also, on a second though, can you prepare a version of this picture without math symbol? all these symbols makes it hard to follow and we need to put the figure at a stage where much of the notation is not introduced yet. same for the test picture}}
% \hc{I used wider colored arrow to emphasize the loop.}
% {\color{orange} SL: we need to use larger font sizes and thicker arrows, use dark blue or grey if you need to use colors.}
% \label{fig:systemOverview}
% \end{figure}


% The flowchart of the testing phase, when we deploy the AP systems with control policy $\controlpolicy$ on patients, is illustrated in Fig~\ref{fig:system_test}. The AP system collects CGM measurements for $\controlpolicy$. $\controlpolicy$ uses CGM measurement history, past insulin injection and future meals and compute the appropriate insulin amount for the patient. A challenge for the test phase is that we does not have access to the state of the patient, but only the subcutaneous glucose level measurements $y_{1,\cdots,t}$ collected by CGM. However, learning optimal actions calculated using full state $x_t$ but train on CGM measurement history, past insulin injection and future meals allows $\controlpolicy$ implicitly learns the mapping from them to $x_t$.

% \begin{figure}[tbp]
% \centerline{\includegraphics[width= 0.3\textwidth]{img/system_test4.PNG}}
% \caption{A virtual patient is using our artificial pancreas system to control blood glucose level in test time. \np{we should put it side-by-side with classical MPC that has state estimation, in order to emphasize our approach}}
% \label{fig:system_test}
% \end{figure}


% % \begin{figure*}[tbp]

% % \begin{subfigure}{0.4\textwidth}
% % \includegraphics[width=\textwidth]{img/system_test4.PNG}
% % \caption{}
% % \label{fig:subim1}
% % \end{subfigure}

% % \begin{subfigure}{0.4\textwidth}
% % \includegraphics[width=\textwidth]{img/system_test_MPC.PNG} 
% % \caption{}
% % \label{fig:subim2}
% % \end{subfigure}

% % \end{figure*}

% % \begin{figure}
% %     \centering
% %     \subfloat{ \includegraphics[width = 0.25\textwidth]{img/system_test4.PNG}}
% %     \subfloat{\includegraphics[width = 0.25\textwidth]{img/system_test_MPC.PNG}}
% % \end{figure}

% We describe and explain the details of the system flowchart and algorithms later in this section. 




% \subsection{Algorithm Description}

% One naive method for a control policy to learn from a computational teacher such as an MPC controller is to generate blood glucose trajectories of patients controlled by the optimal insulin infusion rates computed by the MPC. This trajectory optimization using supervised learning ignores the possibility that the state distributions in the training dataset and test dataset are different~\cite{ross2011reduction}. For a sequence prediction problem like blood glucose control for diabetes patients, errors made in the process will be accumulated and quickly drive the plant system to an unseen state where the control policy is untrained and produce unpredictable outputs.

% We propose an imitation learning algorithm for the AP control policy using adaptive trajectory optimization to explore the state space that the trained control policy is likely to visit in the test time, i.e., the time patient blood glucose is controlled by the control policy. 

% First, we introduce how the supervised policy $\superviseMPC$ computes the optimal control action $\actionSuperviseMPC$ at time $t$. We formulate an optimization problem as the following:

% \begin{align}
% & \underset{u_{t,\ldots,t+\predh-1}}{\min} J = \sum_{k=1}^\predh  d(\tilde{\mathbf{x}}_{t+k}) + \beta\cdot \sum_{k=0}^{\ctrlh - 1} (\Delta u_{t+k})^2 & \label{eq:rob_mpc_prob}
% \end{align}
% \noindent subject to
% \begin{align}
% & u_{t+k} \in D_{u}, \quad k=0,\ldots,\ctrlh -1 \label{eq:rob_mpc2}\\
% & u_{t+k} = \bar{u}, \quad k=\ctrlh,\ldots,\predh -1\label{eq:rob_mpc4}\\
% & \tilde{\bf x}_t = {\bf x}_t \label{eq:rob_mpc5}\\
% & \dot{\tilde{\mathbf{x}}}_{t+k} = F(\tilde{\bf x}_{t+k},u^T_{t+k},\disturbance_{t+k}), \ k=0,\ldots,\predh -1\label{eq:rob_mpc6}
% \end{align}

% where $N_c$ and $N_p$ are the control and prediction horizon (in minutes), respectively. Equation~(\ref{eq:rob_mpc2}) states that the control input $u$ must belong to some set $D_{u}$ of admissible insulin inputs. Equation~(\ref{eq:rob_mpc4}) imposes that $u$ is fixed to the basal insulin rate $\bar{u}$ outside the control horizon. Constraints~(\ref{eq:rob_mpc5}) and (\ref{eq:rob_mpc6}) restrict how the supervised policy $\superviseMPC$ computes the predicted state vector $\tilde{\bf x}$: for the initial state, it uses true state $\mathbf{x}_t$ at time $t$ while subsequent states are predicted using the plant model (\ref{eq:state_space_form}) with insulin dosages $u^T$ from the {\it adaptive teacher policy} $\teacherMPC$. We set control and prediction horizons to $N_c = 100$ min and $N_p = 150$ min, respectively. \np{why we use the adaptive teacher policy in the optimization of the supervision policy? doing so, the optimization variables are unconstrained!!! I don't think that this is what we do}
% \hc{The decision variable in supervision policy is $\actionSuperviseMPC$, in the adaptive teacher policy is $\actionTeacherMPC$}

% The optimization formulation minimizes the summation of two terms:
% \begin{enumerate}
%     \item The sum of Euclidean distances between the predicted BG trajectory and the target BG trajectory:
%     \begin{equation}
%         \sum_{k=1}^\predh  d(\tilde{\mathbf{x}}_{t+k})= \sum_{k=1}^\predh  \gamma_{t+k} 
%         \left(h(\tilde{\mathbf{x}}_{t+k}) - BG^{target}_{t+k}\right)^2
%         \label{eq:traj_discrepancy}
%     \end{equation}
%     where $BG^{target}_{t+k}$ is the target BG at time $t+k$; coefficient $\gamma_{t+k}= \gamma$ if $h(\tilde{\mathbf{x}}_{t+k}) \leq BG^{target}_{t+k}$ and 1 otherwise. We choose $\gamma > 1$ to build an asymmetrical term that is penalized more when the predicted BG is below its corresponding target because asymmetrical cost functions are able to effectively avoid hypoglycemia~\cite{gondhalekar2016periodic}, which could be more dangerous than hyperglycemia. 
%     \item The sum of step-wise difference between consecutive control actions:
%     \begin{equation}
%         \sum_{k=0}^{\ctrlh - 1} (\Delta u_{t+k})^2 = \sum_{k=0}^{\ctrlh - 1} \left( u_{t+k+1} -u_{t+k}\right)^2
%         \label{eq:step_action}
%     \end{equation}
%     This penalize abrupt changes of the insulin infusion rate of the insulin pump.
% \end{enumerate}

% In our setup, We set our target BG trajectory as a steady concentration level of 7.8 mmol/L for all time instants and set penalty coefficient $\beta$ to $0.02$. We set the asymmetric cost penalty $\gamma = 2$.

% Second, we describe the control law used by adaptive teacher policy $\teacherMPC$ at time $t$ to compute its output $\actionTeacherMPC$ using the following optimization formulation:

% \begin{align}\label{eq:teacher_prob}
% & \underset{u_{t,\ldots,{t+\predh-1}}}{\min} J + \rho * J_M
% \end{align}
% \noindent subject to\\
% \begin{equation}
%         J_M = \|\actionTeacherMPC-\controlpolicy(\actionControlpolicy|s^L_t, y_{t},u^T_{t-1},\disturbance_{t+\predh})\|^2\label{eq:match_distribution}
% \end{equation}
% and (\ref{eq:rob_mpc2}), (\ref{eq:rob_mpc4}), (\ref{eq:rob_mpc5}), (\ref{eq:rob_mpc6}). where $\rho$ determines the relative importance of matching the behavior of the learner policy $\controlpolicy$ to minimizing the cost function $J$. We set $\rho = 1- 0.8^{i-1}$ where $i$ is illustrated in algorithm~\ref{alg:1} for that we stress more on the relative importance of matching $\controlpolicy$ as it improves.

% Algorithm~\ref{alg:1} outlines our learning based algorithm for training the artificial pancreas learner policy. The training dataset $S$ is initialized as an empty set. The algorithm runs $N$ iterations of trajectory optimization of length $T$ minutes. At the end of each iteration, the learner policy is trained on the training dataset $S$ with supervised learning methods.

% \hc{TO HERE}
% The learner policy is randomly initialized as $\pi^L_{\theta_1}$ at the beginning of the algorithm. % A meal prediction module is used to predict an estimate of the carbohydrate intake of the patient at time $t+N$ where $N$ is the prediction window of the MPC controllers. At time $t$, we denote $$D_{policy} = (\controlcontext)$$ as {\it control context}, which is the input of the control policy; and $$D_{mpc} = (\traincontext)$$ as {\it training context}, an input for the MPC controllers where $x^t$ is the current patient state, $y^{t-\ctrlh+1},.., y^t$ are the past CGM measurements, $u^{t-\ctrlh+1},..,u^t$ are the past insulin injections and $D_G^t,...,D_G^{t+\predh-1}$ are the future meal predictions.
% At time $t$, the supervised MPC controller $\superviseMPC$ is used to compute the optimal control $\actionSuperviseMPC^t$ to minimize an objective function (\ref{eq:rob_mpc_prob}) under constraints (\ref{eq:rob_mpc2}), (\ref{eq:rob_mpc4}), (\ref{eq:rob_mpc5}), and (\ref{eq:rob_mpc6}).  At time $t$, the teacher MPC controller $\teacherMPC$ interacts with with the current control policy $\controlpolicy^t$ and computes a sub-optimal insulin infusion rate $\actionControlpolicy^t$ for the virtual patients in order to adaptatively minimize the summation of $J$, the trajectory objective and $J_M$, the Euclidean distance between decision control action $u^t$ and the control policy output $\controlpolicy^t(\actionControlpolicy^t|\controlcontext)$. In this way, $\teacherMPC$  will take reasonable and robust actions to visit a similar state space that would likely be seen by control policy $\controlpolicy$. $\teacherMPC$ is not only optimizing the long-term prediction performance during BG control, but also approximating the behavior of $\controlpolicy$. At the end of each iteration, $\controlpolicy$ is trained using training set $S$, improve its control performance and approximating an MPC controller. As a results, the distribution of the patient state in training time will gradually approximate the distribution in test time. 

% At training time, our assumption is the training algorithm is conducted on a simulated virtual patient model, so full information of the patient state is known for both supervised MPC controller $\superviseMPC$ and teacher MPC controller $\controlpolicy$. However, at test time, we assume a more realistic setting: the AP systems do not have access to full information of the patient state, and the only accessible bio-physiological parameter is the subcutaneous glucose measurements collected by CGM sensors. It is challenging to compute the optimal control when only observations (i.e., CGM measurements) that contains partial information of the system state are available to a control policy. To overcome this obstacle, we use full information of the patient states in the MPC controllers, avoiding the estimation of state if only partial state information is available~\cite{paoletti2019data}. On the other hand, we use only observations to train the control policy. One key advantage of our proposal is that in a realistic scenario where only CGM measurements, which are noisy and delay from the blood glucose, of the patient is accessible to the AP, the control policy $\controlpolicy$ is able to learn the process of state estimation implicitly, and map the appropriate insulin injection dosage from the control context, which only contains a series of observations of the test subject. Then the latest CGM measurement $y_t$, latest insulin injection provided to the patient $\actionTeacherMPC$ and meal disturbance $\disturbance_{t+\predh}$ will be collected as the training inputs of $S$. The corresponding training output is the optimal insulin amount $u_S^t$ will be collected into the training dataset $S$. At time $t$, the CGM collects the subcutaneous glucose measurement $y_t$ of the patient. 





% \begin{algorithm}[tbp]\label{alg:1}
% \SetAlgoLined

%  Initialize data $S\leftarrow \emptyset$\;
%  Randomly initialize learner policy $\pi^L_{\theta_1}$\;
%  \For{$i=1$ to $N$}{
%  Randomly initialize the patient state\;
%   \For{$t=1$ to $T$}{
%   Access the full state of the patient model  $x_t$\;
%   Gain CHO amount of meal $\disturbance_{t+\predh}$\;
%   Compute optimal insulin dosage $\actionSuperviseMPC$ with supervised policy $\superviseMPC(\actionSuperviseMPC|x_t, d_{t,\cdots,t+\predh})$ by solving optimization problem~(\ref{eq:rob_mpc_prob}), subject to constraints~(\ref{eq:rob_mpc2}), (\ref{eq:rob_mpc4}), (\ref{eq:rob_mpc5}), and (\ref{eq:rob_mpc6}) \label{lst:line:teacher_policy}\;
%   Collect CGM measurements $y_t$\;
%   Compute sub-optimal insulin dosage $\actionTeacherMPC$ with adaptive teacher policy $\teacherMPC(\actionTeacherMPC|x_t,d_{t,\cdots,t+\predh}, \controlpolicy)$ by solving optimization problem~(\ref{eq:teacher_prob}), subject to constraints~(\ref{eq:rob_mpc2}), (\ref{eq:rob_mpc4}), (\ref{eq:rob_mpc5}), and (\ref{eq:rob_mpc6})\label{lst:line:supervision_policy}\;
%   Append $(\{y_t,\actionTeacherMPC,d_{t+\predh\}},\actionSuperviseMPC)$ to $S$ \label{lst:line:supervised_action}\;
%   State evolve for the patient $x_{t+1} =  {\bf F}\left(\mathbf{x}_t, \actionTeacherMPC, \disturbance_t \right)$\label{lst:line:evolve_by_teacher} 
%   }
%   Train $\pi^L_{\theta_{i+1}}$ on $S$\label{lst:line:train_by_supervision}
%  }
%  \caption{artificial pancreas control policy training algorithm using adaptive trajectory optimization}
% \end{algorithm}

% \subsection{Bayesian recurrent neural network}

% \hc{We need some theoretical insight to prove this method other than a best practice. Maybe dropout can approximate a deep Gaussian process and our model parameters are Gaussian? We need to see more into~\cite{gal2016dropout}}.

% A major challenge to manage a type 1 diabetes patients' BG in healthy range is the uncertainty of external disturbance, i.e., CHO ingestion. Another major challenge is the intra-patient variation of a single patient which is the phenomena that the insulin-glucose regulatory metabolism of that patient has minor variations that are hard to detect. To mitigate these challenges, we introduce model uncertainty into the our neural network control policy by employing dropout in both training and testing to approximate a Bayesian neural network. In~\cite{gal2016dropout}, the paper proved that a neural network of any architecture with dropout applied before every weighted layer is mathematically equivalent to an approximation
% of a probabilistic deep Gaussian process. 

% In a {\it standard dropout} layer with dropout probability $p$, at training time, the neurons are randomly dropped and set to zero with probability $p$. At test time, a standard dropout multiplies each hidden unit with a factor of $1/(1-p)$ to scale back the outputs. By employ the mechanism of randomly drop neurons and set them to zero in both training and testing, it utilizes outputs from the network with different parameters to do uncertainty estimation in order to tune the neural network hyper-parameters and reduce the generalization error.

% Using this variant of dropout layer that enable dropout at test time, it is shown that multiple outputs generated from the same network using the same input multiple times are equivalent to the results of Monte-Carlo sampling~\cite{gal2016dropout}. At time $t$, the control policy $\controlpolicy$ makes $T$ stochastic forward passes and computes an output using the following equation: 
% \begin{equation}\label{eq:stochatic_strategy}
% \actionControlpolicy^t = g(\actionControlpolicy^{t_1},...,\actionControlpolicy^{t_T})
% \end{equation}
%  with some integration strategy $g$. With this important feature, our control policy has the potential to improve its ability to generalize it control capability from one static patient to a patient with intra-patient variation and even to a patient cohort. it also has generalization property for different meal distributions that are unseen in the training data. 

% At time $t$, the stochastic control policy has a distribution $q(\actionControlpolicy|D_{policy})$ over output instead of a deterministic output. We rewrite (\ref{eq:match_distribution}) using the $p$-th Wasserstein distance, which defined as a distance function of two probability distributions on a given metric space $M$:
% \begin{align}
%         J_M = &  W_p\left(p(\actionTeacherMPC|D_{mpc}),q(\actionControlpolicy|D_{policy})\right) \\
%         = & \underset{\gamma \in \Gamma(\actionTeacherMPC,\actionControlpolicy)}{\inf}\left(\int_{M\times M}d(\actionTeacherMPC,\actionControlpolicy)^p d\gamma(\actionTeacherMPC,\actionControlpolicy)\right)^{1/p}\\
%         = & \inf (E[d(\actionTeacherMPC,\actionControlpolicy)^p])^{1/p}
%         \label{eq:wasserstein_metric}
% \end{align}

% In our case, $p$ is a Dirac delta distribution and $q$ is approximately a Gaussian distribution. We choose Wasserstein distance as our measure metric because $p$ and $q$ are likely to have disjoint supports, many other common distance or divergence (e.g., Kullback–Leibler divergence) is possibly undefined or simply infinite~\cite{arjovsky2017wasserstein}.
% In the optimization at time $t$, we use sampling to compute empirical distributions $p$ and $q$ and approximate $J_M$ with compositions of delta functions. We assume $q \approx \frac{1}{n}\sum_{i=1}^n \delta_{x_i}$ and $p \approx \frac{1}{n}\sum_{i=1}^n \delta_{y_i}$, where $x_i$ and $y_i$ are not unique. $J_m$ has an approximation:
% \begin{equation}
%     \begin{split}
%             J_M & \approx  W_p\left(\frac{1}{n}\sum_{i=1}^n \delta_{x_i},\frac{1}{n}\sum_{i=1}^n \delta_{y_i}\right)\\
%   & =  \underset{\sigma_i\in S_n}{\min}\sum_{i=1}^n(d(y_i, x_{\sigma_i})^p)^{1/p}\\
%   & = \left(\sum_{i=1}^T d(\actionTeacherMPC^t, \actionControlpolicy^{t_i})^p\right)^{1/p}\\
%   & = \left(\sum_{i=1}^T ||\actionTeacherMPC^t- \actionControlpolicy^{t_i}||_2\right)^{1/2}
%     \end{split}
% \end{equation}

% Note that the Wasserstein distance of two Dirac delta distributions is the following:
% \begin{equation}
%     W_p(u_1,u_2) = ||a_1-a_2||_2,
% \end{equation}
% where $u_1 = \delta_{a_1}, u_2 = \delta_{a_2} \in \mathbb{R}^n$, if we use the Euclidean norm as the distance function. So (\ref{eq:match_distribution}) is also a special case of Wasserstein distance.


% % \subsection{Online retraining}

% % The inter-patient variation, in which the metabolisms among different patients in a patient cohort are individually different, is huge challenge for the BG control for type 1 diabetes. One control policy that performance well on one patient is likely to act worse on another. We propose an online retraining for the control policy to keep learning new physiological information of the patient that wears an artificial pancreas system. Algorithm~\ref{alg:2} illustrates the retraining scheme.

% % After we train the control policy $\controlpolicy$, the AP system controlled by $\controlpolicy$ is applied on a virtual test patient. The stochastic strategy is trying to generate an output $\actionControlpolicy^t$ that uses the hyper-parameterization of neural network that best capture the new patient model's parameter information. The data samples are collected into the training set and $\controlpolicy$ is trained every same time interval $T_i$. 

% % \begin{algorithm}[tbp]\label{alg:2}
% % \SetAlgoLined

% %  Initialized dataset $S_{online}\leftarrow S$\
 
% % \For{$t=1$ to $T$}{
% %   Use control policy $\controlpolicy$ to make $T$ stochastic forward passes $\actionControlpolicy^{t_1},...,\actionControlpolicy^{t_T}$\;
% %   Compute output $\actionControlpolicy^t = g(\actionControlpolicy^{t_1},...,\actionControlpolicy^{t_T})$ using some function $g$\;
% %   Append $(D_{policy},\actionControlpolicy^t)$ to $S$ \label{lst:line:supervised_action}\;
% %     State evolve $x(t+1) =  {\bf F}\left(\mathbf{x}(t), u^t, D_G^t \right)$\label{lst:line:evolve_by_teacher} \;
% %   \uIf{$t$ mod $T_i = 0$}{
% %   Train $\pi_\theta$ on $S$\label{lst:line:train_by_supervision}\;
% %   }
% %   }
 
% %  \caption{Online retraining for control policy}
% % \end{algorithm}
